An artifcial life approach to studying niche differentiation in soundscape ecology

Artificial life simulations are an important tool in the study of ecological phenomena that can be difficult to examine directly in natural environments. Recent work has established the soundscape as an ecologically important resource and it has been proposed that the differentiation of animal vocalizations within a soundscape is driven by the imperative of intraspecies communication. The experiments in this paper test that hypothesis in a simulated soundscape in order to verify the feasibility of intraspecies communication as a driver of acoustic niche differentiation. The impact of intraspecies communication is found to be a significant factor in the division of a soundscape's frequency spectrum when compared to simulations where the need to identify signals from conspecifics does not drive the evolution of signalling. The method of simulating the effects of interspecies interactions on the soundscape is positioned as a tool for developing artificial life agents that can inhabit and interact with physical ecosystems and soundscapes.

==> sections/notes.tex <==
What is my null model? \citep[p5]{Eldridge2018}

\citep{Eldridge2018} answer a bunch of the basic questions:
\begin{itemize}
	\item Do patterns emerge over time
	\item Population recovery after noise
	\item The advantage of coherent communication
	\item Variation of complexity measures over the course of the run
	\item Temporal and spectral effects
	\item Full model of reproduction, energetic effects, etc.
\end{itemize}

There are some differences:
\begin{itemize}
	\item I am asking the receiver to reproduce a full message, which they aren't
	\item I can look at brain size/complexity with number of species
	\item I am looking at multiple "frequencies", so I can look at message complexity...
	\item NEURO! I can look at brain. They are evolving parameters...
	\item How the addition of species affects brain complexity...
	\item They don't add an extra species.
	\item They have single agents representing a population. I can look at intra-species diversity and how that changes during a disturbance...
\end{itemize}

Some questions I can ask:
\begin{itemize}
	\item \sout{How does speciation (in NEAT) affect the success rates and fitness?}
	\item How different are the signals from the two groups over time (intraspecies vs interspecies)
	\item How does brain complexity change based on trajectory (how many species to start), number of species, type of interference (new coherent species, random species, random noise)? How does response and resulting spectrum differ based on that?
	\item How does a separable vs non-separable space differ?
	\item How does complexity of the encoder relate to complexity of the decoder?
	\item How does the cost of a frequency drive the elimination of certain bands? (Energetic cost)...
	\item Could you drive the adoption of a particular frequency among a species by repeating sounds in that band?
\end{itemize}

How is the niche conceptualized as a behavioural vs evolutionary artifact...

==> sections/outline.tex <==
Outline:
\begin{enumerate}
	\item Introduction
	\begin{itemize}
		\item Problem: Can computational evolution be used to probe the mechanisms behind the ANH?
		\item Theoretical Framework: ALife --- computational explorations of artificial life-like forms --- can help allow rapid experimentation with evolutionary processes
		\item Methodology: Evolve populations with fitness tied to the identification of co-specific members and the decoding of messages, and assess the divergence of messages and spectral use.
		\item Hypothesis: Populations will tend towards the use of non-overlapping frequency bands for their messages. More successful populations will use fewer overlapping bands. \\
			Under evolutionary pressure to communicate within their own species, communities will tend to divide a frequency spectrum so as to not overlap their signals. \\
			Those that divide more successfully are better communicators. And that are closest in their internal signals
		\item Review: \citet{Krause1987} for ANH, \citet{Pijanowski2011a} for soundscape ecology, and \citet{Eldridge2018} for synthetic acoustic ecology
		\item Scope: Only spectral...not looking at timing. Looking at 9 bands, roughly representing 9 frequencies. Not accounting for morphology (MAH), spatiality, etc. Toy set.
		\item Significance: It is a toy set from which more studies can be built to look at intra-population diversity as well as inter-population diversity. Can look at priority effects, etc.
	\end{itemize}
	\item Background
	\begin{itemize}
		\item \citet{Krause1987} proposes \gls{anh} as a way of describing how acoustic signatures of ecosystems are formed. Proposes that one can judge the health/age of an ecosystem by sound.
		\item \citep{Boncoraglio2007} has some criticisms. Are they correct?
		\item \citet{Pijanowski2011a} discusses \gls{anh} as a part of the new field of soundscape ecology
		\item \citet{Eldridge2018} describes synthetic acoustic ecology as a mode of rapid exploration of the evolution of soundscape ecologies
		\item This work extends the work of \citet{Eldridge2018} by moving the evolution into a neural context and allowing intraspecific diversity as well as interspecific diversity.
		\item This allows for the study of how populations incorporate genetic innovations over time so as to occupy new niches. It also allows us to understand the \textbf{impulse response} of the system so that we can understand what might happen when introducing a new sound source into an ecosystem.
	\end{itemize}
	\item Methods
	\begin{itemize}
		\item \gls{sac}
		\item \gls{neat}
		\item simplified "sonic space"
		\item ignoring temporal effects
		\item ignoring the cost of sound production and negative evolutionary pressures
	\end{itemize}
	\item Results
	\begin{itemize}
		\item 
	\end{itemize}
	\item Discussion
	\begin{itemize}
		\item 
	\end{itemize}
	\item Conclusions
	\begin{itemize}
		\item 
	\end{itemize}
\end{enumerate}
